Unsupervised Learning of Disentangled Representations from Video

We present a new model DrNET that learns disentangled image representations from video. Our approach leverages the temporal coherence of video and a novel adversarial loss to learn a representation that factorizes each frame into a stationary part and a temporally varying component. The disentangled representation can be used for a range of tasks. For example, applying a standard LSTM to the time-vary components enables prediction of future frames. We evaluate our approach on a range of synthetic and real videos, demonstrating the ability to coherently generate hundreds of steps into the future.

==> model.tex <==

\section{Model architectures}

%\subsection{KTH Action Dataset}
%For this we used a U-Net architecture \cite{ronneberger2015u}, based around the
%VGG model \cite{vgg}. 

\textbf{VGG16 Encoder}

//$conv1:128 \rightarrow 64$\\
conv(64) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(64) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
pool 2x2\\
// $conv2: 64 \rightarrow 32$\\
conv(128) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(128) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
//$conv3: 32 \rightarrow 16$\\
conv(256) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(256) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(256) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
pool 2x2\\
//$conv4: 16 \rightarrow 8$\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
pool 2x2\\
//$conv5: 8 \rightarrow 4$\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
pool 2x2\\
//$conv6: 4 \rightarrow 1$\\
conv($\left\vert{h}\right\vert $) 4x4 $\rightarrow$ batchnorm $\rightarrow$ tanh $\rightarrow$ normalize  \\


\textbf{VGG16 Decoder}\\
//$upconv1: 1 \rightarrow 4$\\
upconv(512) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
//$upconv2: 4 \rightarrow 8$\\
upsamplenearest2\\
upconv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
//$upconv3: 8 \rightarrow 16$\\
upsamplenearest2\\
conv(512) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(256) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
//$upconv4: 16 \rightarrow 32$\\
upsamplenearest2\\
conv(128) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(64) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
//$upconv5: 32 \rightarrow 64$\\
upsamplenearest2\\
conv(64) 3x3 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(numcolor ) 3x3 $\rightarrow$ sigmoid\\
//$upconv6: 64 \rightarrow 128$ $\rightarrow$ sigmoid\\

For U-Net model, we have skip connections between:
$conv2 \rightarrow upconv5$\\
$conv3 \rightarrow upconv4$\\
$conv4 \rightarrow upconv3$\\
$conv5 \rightarrow upconv2$\\

\textbf{DCGAN Encoder}

conv(64) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(128) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(256) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(512) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv($\left\vert{h}\right\vert $) 4x4 $\rightarrow$ batchnorm $\rightarrow$ tanh $\rightarrow$ normalize  \\



\textbf{DCGAN Decoder}

conv(512) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(256) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(128) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(64) 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv32 4x4 $\rightarrow$ batchnorm $\rightarrow$ leaky relu\\
conv(numcolor ) 3x3 $\rightarrow$ sigmoid\\




\subsection{Forward Model architectures}
Forward model: LSTM with 2 layers, 256 cells per layer, trained on seqeunces of length 20. At each time step the LSTM gets the same content vector (extracted from the last conditioned frame) and the pose vector for the time step. 

